LoRA Land: 310 Fine-tuned LLMs that Rival GPT-4, A Technical Report

Low Rank Adaptation (LoRA) has emerged as one of the most widely adopted methods for Parameter Efficient Fine-Tuning (PEFT) of Large Language Models (LLMs). LoRA reduces the number of trainable parameters and memory usage while achieving comparable performance to full fine-tuning. We aim to assess the viability of training and serving LLMs fine-tuned with LoRA in real-world applications. First, we measure the quality of LLMs fine-tuned with quantized low rank adapters across 10 base models and 31 tasks for a total of 310 models. We find that 4-bit LoRA fine-tuned models outperform base models by 34 points and GPT-4 by 10 points on average. Second, we investigate the most effective base models for fine-tuning and assess the correlative and predictive capacities of task complexity heuristics in forecasting the outcomes of fine-tuning. Finally, we evaluate the latency and concurrency capabilities of LoRAX, an open-source Multi-LoRA inference server that facilitates the deployment of multiple LoRA fine-tuned models on a single GPU using shared base model weights and dynamic adapter loading. LoRAX powers LoRA Land, a web application that hosts 25 LoRA fine-tuned Mistral-7B LLMs on a single NVIDIA A100 GPU with 80GB memory. LoRA Land highlights the quality and cost-effectiveness of employing multiple specialized LLMs over a single, general-purpose LLM.

==> tables/base_models_performance.tex <==
% \begin{landscape}
\begin{table}[]
\label{table:basemodelsperformance}
\centering
\scalebox{0.5}{

\begin{tabular}{ccccccccccccccc}

\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Metric}} & \textbf{Microsoft} & \multicolumn{4}{c}{\textbf{Google}}                                                             & \multicolumn{2}{c}{\textbf{Meta}}              & \multicolumn{2}{c}{\textbf{Mistral}}               & \textbf{Hugging Face}   & \multicolumn{2}{c}{\textbf{OpenAI}}     \\
                                   &                                &                                  & \textbf{phi-2}     & \textbf{gemma-2b} & \textbf{gemma-2b-instruct} & \textbf{gemma-7b} & \textbf{gemma-7b-instruct} & \textbf{llama-2-7b} & \textbf{llama-2-7b-chat} & \textbf{mistral-7b} & \textbf{mistral-7b-instruct} & \textbf{zephyr-7b-beta} & \textbf{gpt-3.5-turbo} & \textbf{gpt-4} \\
\multirow{7}{*}{Classic NLP}       & bc5cdr                         & rouge                            & 0.172              & 0.013             & 0.494                      & 0.075             & 0.198                      & 0.185               & 0.024                    & 0.177               & 0.703                        & 0.146                   & 0.732                  & \textbf{0.890} \\
                                   & conllpp                        & rouge                            & 0.101              & 0.011             & 0.647                      & 0.085             & 0.120                      & 0.108               & 0.115                    & 0.148               & 0.733                        & 0.088                   & \textbf{0.810}         & 0.742          \\
                                   & e2e\_nlg                       & rouge                            & 0.132              & 0.174             & 0.281                      & 0.152             & 0.434                      & 0.087               & 0.442                    & 0.167               & 0.482                        & 0.122                   & 0.467                  & \textbf{0.513} \\
                                   & tldr\_content\_gen             & rouge                            & 0.158              & 0.117             & 0.160                      & 0.089             & 0.141                      & 0.148               & 0.183                    & 0.153               & 0.163                        & 0.164                   & 0.173                  & 0.125          \\
                                   & tldr\_headline\_gen            & rouge                            & 0.169              & 0.034             & 0.155                      & 0.063             & 0.152                      & 0.078               & 0.174                    & 0.071               & 0.171                        & 0.120                   & \textbf{0.195}         & 0.175          \\
                                   & viggo                          & rouge                            & 0.133              & 0.093             & 0.237                      & 0.123             & 0.313                      & 0.141               & 0.356                    & 0.044               & 0.374                        & 0.193                   & 0.372                  & \textbf{0.374} \\
                                   & webnlg                         & rouge                            & 0.120              & 0.055             & 0.312                      & 0.257             & 0.453                      & 0.148               & 0.563                    & 0.091               & 0.541                        & 0.512                   & 0.581                  & \textbf{0.583} \\
\multirow{2}{*}{Coding}            & magicoder                      & humaneval                        & 0.012              & 0.037             & 0.024                      & 0.030             & 0.018                      & 0.012               & 0.134                    & 0.201               & 0.152                        & 0.049                   & 0.683                  & \textbf{0.829} \\
                                   & wikisql                        & rouge                            & 0.143              & 0.030             & 0.301                      & 0.036             & 0.244                      & 0.043               & 0.093                    & 0.265               & 0.134                        & 0.080                   & 0.887                  & \textbf{0.909} \\
\multirow{8}{*}{Knowledge}         & boolq                          & accuracy                         & 0.691              & 0.447             & 0.661                      & 0.300             & 0.735                      & 0.645               & 0.759                    & 0.669               & 0.764                        & 0.683                   & 0.870                  & \textbf{0.911} \\
                                   & dbpedia                        & dbpedia                          & 0.268              & 0.018             & 0.086                      & 0.021             & 0.089                      & 0.043               & 0.868                    & 0.036               & 0.313                        & 0.578                   & 0.853                  & \textbf{0.965} \\
                                   & customer\_support              & accuracy                         & 0.250              & 0.120             & 0.380                      & 0.100             & 0.850                      & 0.110               & 0.630                    & 0.030               & 0.730                        & 0.540                   & \textbf{1.000}         & \textbf{1.000} \\
                                   & glue\_qnli                     & accuracy                         & 0.496              & 0.439             & 0.444                      & 0.463             & 0.685                      & 0.510               & 0.736                    & 0.533               & 0.743                        & 0.569                   & 0.829                  & \textbf{0.902} \\
                                   & glue\_stsb                     & mae                              & 0.682              & 0.197             & 0.590                      & 0.537             & 0.729                      & 0.651               & 0.680                    & 0.672               & 0.723                        & 0.814                   & \textbf{0.857}         & 0.773          \\
                                   & legal                          & rouge                            & 0.008              & 0.010             & 0.037                      & 0.019             & 0.053                      & 0.009               & 0.026                    & 0.001               & 0.158                        & 0.039                   & 0.266                  & \textbf{0.305} \\
                                   & reuters                        & rouge                            & 0.003              & 0.001             & 0.010                      & 0.001             & 0.009                      & 0.003               & 0.010                    & 0.004               & 0.010                        & 0.005                   & \textbf{0.026}         & 0.014          \\
                                   & mmlu                           & accuracy                         & 0.339              & 0.160             & 0.279                      & 0.302             & 0.460                      & 0.189               & 0.349                    & 0.402               & 0.446                        & 0.506                   & 0.504                  & \textbf{0.774} \\
\multirow{13}{*}{Reasoning}        & winogrande                     & accuracy                         & 0.380              & 0.309             & 0.515                      & 0.390             & 0.576                      & 0.503               & 0.515                    & 0.498               & 0.546                        & 0.532                   & 0.569                  & \textbf{0.832} \\
                                   & arc\_combined                  & accuracy                         & 0.323              & 0.180             & 0.254                      & 0.272             & 0.657                      & 0.304               & 0.379                    & 0.573               & 0.673                        & 0.497                   & 0.926                  & \textbf{0.947} \\
                                   & glue\_cola                     & accuracy                         & 0.463              & 0.152             & 0.642                      & 0.062             & 0.749                      & 0.691               & 0.691                    & 0.691               & 0.797                        & 0.788                   & 0.843                  & \textbf{0.864} \\
                                   & glue\_mnli                     & accuracy                         & 0.328              & 0.053             & 0.347                      & 0.213             & 0.272                      & 0.315               & 0.293                    & 0.327               & 0.455                        & 0.348                   & 0.588                  & \textbf{0.803} \\
                                   & glue\_mrpc                     & accuracy                         & 0.652              & 0.265             & 0.664                      & 0.654             & 0.652                      & 0.679               & 0.674                    & 0.684               & 0.694                        & 0.676                   & 0.689                  & \textbf{0.777} \\
                                   & glue\_qqp                      & accuracy                         & 0.327              & 0.138             & 0.337                      & 0.316             & 0.396                      & 0.345               & 0.340                    & 0.327               & 0.708                        & 0.340                   & 0.830                  & \textbf{0.841} \\
                                   & glue\_sst2                     & accuracy                         & 0.487              & 0.407             & 0.719                      & 0.187             & 0.682                      & 0.306               & 0.695                    & 0.115               & 0.933                        & 0.706                   & 0.933                  & \textbf{0.942} \\
                                   & glue\_wnli                     & accuracy                         & 0.437              & 0.183             & 0.437                      & 0.366             & 0.437                      & 0.423               & 0.437                    & 0.437               & 0.437                        & 0.437                   & 0.521                  & \textbf{0.930} \\
                                   & covid                          & accuracy                         & 0.207              & 0.154             & 0.317                      & 0.169             & 0.322                      & 0.162               & 0.212                    & 0.191               & 0.297                        & 0.243                   & \textbf{0.334}         & 0.309          \\
                                   & hellaswag                      & accuracy                         & 0.371              & 0.117             & 0.023                      & 0.112             & 0.201                      & 0.381               & 0.264                    & 0.246               & 0.249                        & 0.393                   & 0.622                  & \textbf{0.805} \\
                                   & hellaswag\_processed           & rouge                            & 0.037              & 0.056             & \textbf{0.146}             & 0.109             & 0.143                      & 0.044               & 0.089                    & 0.038               & 0.134                        & 0.040                   & 0.140                  & 0.134          \\
                                   & jigsaw                         & accuracy                         & 0.491              & 0.490             & 0.482                      & 0.233             & 0.520                      & 0.486               & 0.545                    & 0.475               & 0.704                        & 0.472                   & 0.735                  & \textbf{0.754} \\
                                   & drop                           & rouge                            & 0.018              & 0.013             & 0.034                      & 0.024             & 0.042                      & 0.010               & 0.047                    & 0.011               & 0.066                        & 0.023                   & 0.119                  & \textbf{0.393} \\
Math                               & gsm8k                          & accuracy                         & 0.083              & 0.026             & 0.082                      & 0.039             & 0.364                      & 0.051               & 0.160                    & 0.114               & 0.275                        & 0.133                   & \textbf{0.622}         & 0.373         
\end{tabular}
}

\vspace{10mm}
\caption{Model performance for every task and base model.}

\end{table}
